Cops and Robbers on Intersection Graphs

The cop number of a graph $G$ is the smallest $k$ such that $k$ cops win the game of cops and robber on $G$. We investigate the maximum cop number of geometric intersection graphs, which are graphs whose vertices are represented by geometric shapes and edges by their intersections. We establish the following dichotomy for previously studied classes of intersection graphs: The intersection graphs of arc-connected sets in the plane (called string graphs) have cop number at most 15, and more generally, the intersection graphs of arc-connected subsets of a surface have cop number at most $10g+15$ in case of orientable surface of genus $g$, and at most $10g'+15$ in case of non-orientable surface of Euler genus $g'$. For more restricted classes of intersection graphs, we obtain better bounds: the maximum cop number of interval filament graphs is two, and the maximum cop number of outer-string graphs is between 3 and 4. The intersection graphs of disconnected 2-dimensional sets or of 3-dimensional sets have unbounded cop number even in very restricted settings. For instance, we show that the cop number is unbounded on intersection graphs of two-element subsets of a line, as well as on intersection graphs of 3-dimensional unit balls, of 3-dimensional unit cubes or of 3-dimensional axis-aligned unit segments.

==> preliminaries.tex <==
\section{Definitions and Preliminaries}

Let $G = (V,E)$ be a graph.  For a vertex $v$, we use the \emph{open neighborhood} $N(v) = \{u : uv
\in E\}$ and the \emph{closed neighborhood} $N[v] = N(v) \cup \{v\}$. Similarly for $V' \subseteq
V$, we put $N[V']= \bigcup_{v \in V'}N[v]$ and $N(V') = N[V'] \setminus V'$. For $V'\subseteq V$, we
denote by $G|_{V'}$ the subgraph of $G$ induced by $V'$.

\heading{Intersection Representations.}
An \emph{intersection representation} of $G$ is a map $\varphi:V \to 2^X$ for some ground set $X$
such that the edges of $G$ are prescribed by intersections of the sets $\varphi(v)$; formally,
$uv\in E$ if and only if $\varphi(u)\cap\varphi(v)\neq\emptyset$. Given the (multi)set of the images
of $\varphi$, the corresponding \emph{intersection graph} is uniquely defined up to isomorphism.

The ground set $X$ and the images of $\varphi$ are usually somehow restricted to get
a particulate intersection graph family. For example, to get the well-known class of interval graphs,
let $X=\R$ and require every $\varphi(v)$ to be a closed interval.

A \emph{string graph} is an intersection graph of a set of \emph{strings}. We let $X=\R^2$ and
every $\varphi(v)$ is required to be a finite curve, in this context called a string,
that is a continuous image of the interval $[0,1]$ to $\R^2$.

We also study a subclass of string graphs called \emph{interval filament graphs}. An interval filament
graph is a string graph such that each \emph{interval filament} $\varphi(v)$ is a continuous
($x$-monotone) function defined on $[a,b]$ such that $\varphi(v)(a)=\varphi(v)(b) = 0$ and
$\varphi(v)(x) > 0$ for all $x \in (a,b)$. This class was introduced by Gavril~\cite{gavril} as a
generalisation of interval graphs on which his algorithm for weighted maximum clique/independent set
can be used. The connection with interval graphs is as follows: Let $\varphi(u)$ is a filament
defined on $[a,b]$ and $\varphi(v)$ be filament defined on $[c,d]$. If the intervals $[a,b]$ and
$[c,d]$ are disjoint, then $\varphi(u)$ cannot intersect $\varphi(v)$. If the intervals single
overlaps, e.g. $a < c < b < d$, then the filaments have to intersect. But if one interval is
contained inside the other interval, e.g, $a < c < d < b$, then there the filaments $\varphi(u)$ and
$\varphi(v)$ might or might not intersect. (Unlike in interval graphs where the edge/non-edge $uv$
depends only on intersection of $[a,b]$ and $[c,d]$.)

\heading{Assumptions on Representations.}
Let $\varphi:V\to 2^{\R^2}$ be a string representation of $G$. Without loss of generality, we may
assume that there is only a finite number of string intersections in the representation, that
strings never only touch without either also crossing each other or at least one of them ending,
that no three or more strings meet at the same point and that no string self-intersects.  This
follows from the fact that strings are compact subsets of the plane and as such can replaced by
piece-wise linear curves with finite numbers of linear segments, for more details see~\cite{KGK}.
We always assume these properties.

\heading{Regions.}
For a $V'\subseteq V$, let $\varphi(V')=\bigcup_{v\in V'}\varphi(v)$.
Then $\varphi(V')$ divides $\R^2$ into one or more \emph{open regions} which are the connected sets
of $\R^2 \setminus \varphi(V')$. Let $\A(\varphi(V'))$ be the set of these regions. Since we assume
there are finitely many intersections, the set $\A(\varphi(V'))$ is always finite throughout this paper.
Let $\C(X)$ denote the topological closure of a set $X$. We mostly use this operator
on elements of some $\A(\varphi(V'))$ to include the bounding curves.

\heading{Meetings.}
Let $\pi_1$ and $\pi_2$ be curves (as continuous functions from $[0,1]$).
A \emph{meeting} of these curves are intervals $I_1,I_2\subseteq[0,1]$
such that $\pi_1[I_1]=\pi_2[I_2]$ and this intersection has non-zero length.
$\pi_1$ and $\pi_2$ meet if they have at least one meeting. Note that one-point intersection
(crossing) of curves is not a meeting.



